Stationary Distribution of a Generalized LRU-MRU Content Cache

Many different caching mechanisms have been previously proposed, exploring different insertion and eviction policies and their performance individually and as part of caching networks. We obtain a novel closed-form stationary invariant distribution for a generalization of LRU and MRU caching nodes under a reference Markov model. Numerical comparisons are made with an "Incremental Rank Progress" (IRP a.k.a. CLIMB) and random eviction (a.k.a. random replacement) methods under a steady-state Zipf popularity distribution. The range of cache hit probabilities is smaller under MRU and larger under IRP compared to LRU. We conclude with the invariant distribution for a special case of a random-eviction caching tree-network and associated discussion.

==> define.tex <==
\def\IEEEproof{proof}
\def\E{{\sf E}}
\def\P{{\sf P}}
\def\uu{\underline{u}}
\def\utheta{\underline{\theta}}
\def\upi{\underline{\pi}}
\def\uzero{\underline{0}}
\def\uone{\underline{1}}
\def\ugamma{\underline{\gamma}}
\def\ulambda{\underline{\lambda}}
\def\uGamma{\underline{\Gamma}}
\def\uLambda{\underline{\Lambda}}
\def\blambda{\tilde{\lambda}}
\def\bLambda{\tilde{\Lambda}}
\def\ur{\underline{r}}
\def\Rcal{\mathcal{R}}
\def\Ncal{\mathcal{N}}
\def\tP{\tilde{P}}
\def\eg{{\em e.g.},~}
\def\ie{{\em i.e.},~}
\def\cf{{\em cf.},~}
\newtheorem{proposition}{Proposition}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newcommand{\beqa}{\begin{eqnarray*}}
\newcommand{\eeqa}{\end{eqnarray*}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}

\renewcommand{\th}[1]{{#1}^{\rm th}}
\newcommand{\rinv}[1]{r^{-1}(#1)}
\newcommand{\Sinv}[1]{S^{-1}_{#1}}
\newcommand{\Minv}[1]{M^{-1}_{#1}}
\newcommand{\Tinv}[1]{T^{-1}_{#1}}
\newcommand{\Hinv}[1]{H^{-1}_{#1}}

